A general randomized test for Alpha

We propose a methodology to construct tests for the null hypothesis that the pricing errors of a panel of asset returns are jointly equal to zero in a linear factor asset pricing model -- that is, the null of "zero alpha". We consider, as a leading example, a model with observable, tradable factors, but we also develop extensions to accommodate for non-tradable and latent factors. The test is based on equation-by-equation estimation, using a randomized version of the estimated alphas, which only requires rates of convergence. The distinct features of the proposed methodology are that it does not require the estimation of any covariance matrix, and that it allows for both N and T to pass to infinity, with the former possibly faster than the latter. Further, unlike extant approaches, the procedure can accommodate conditional heteroskedasticity, non-Gaussianity, and even strong cross-sectional dependence in the error terms. We also propose a de-randomized decision rule to choose in favor or against the correct specification of a linear factor pricing model. Monte Carlo simulations show that the test has satisfactory properties and it compares favorably to several existing tests. The usefulness of the testing procedure is illustrated through an application of linear factor pricing models to price the constituents of the S&P 500.

==> Tables/tab_MC_FM.tex <==
\begin{tabular}{l|ccccccccccc}
\toprule
&\multicolumn{10}{c}{Gaussian noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.041 & 0.033 & 0.025 & 0.028 & 0.024 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.048 & 0.037 & 0.038 & 0.027 & 0.045 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.043 & 0.039 & 0.033 & 0.045 & 0.032 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{Student's $t$ noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.026 & 0.033 & 0.034 & 0.037 & 0.022 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.035 & 0.032 & 0.040 & 0.033 & 0.038 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.058 & 0.040 & 0.030 & 0.038 & 0.040 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{GARCH noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.055 & 0.045 & 0.032 & 0.035 & 0.043 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.081 & 0.037 & 0.042 & 0.025 & 0.019 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.091 & 0.038 & 0.040 & 0.036 & 0.045 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\bottomrule
\end{tabular}


==> Tables/tab_MC_PCA.tex <==
\begin{tabular}{l|ccccccccccc}
\toprule
&\multicolumn{10}{c}{Gaussian noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100 &0.047 &0.033 &0.025 &0.028 &0.024 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.052 &0.037& 0.038 &0.027 &0.045 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.050 &0.040 &0.033 &0.045& 0.032 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{Student's $t$ noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.033 &0.032& 0.033& 0.033 &0.022 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.042 &0.033& 0.041& 0.032 &0.038 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.065 &0.040& 0.030 &0.038 &0.041 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{GARCH noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.080 &0.047 &0.030& 0.034 &0.043&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.131& 0.051 &0.043& 0.027 &0.019&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500 &0.193& 0.064& 0.049& 0.039 &0.046&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\bottomrule
\end{tabular}








==> Tables/tab_MC_PCAbis.tex <==
\begin{tabular}{l|ccccccccccc}
\toprule
&\multicolumn{10}{c}{Gaussian noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.043 & 0.032 & 0.025 & 0.07 & 0.024 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.050 & 0.037 & 0.039 & 0.027 & 0.045 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.047 & 0.042 & 0.033 & 0.044 & 0.033 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{Student's $t$ noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100& 0.040 &0.033 &0.032 &0.033& 0.022&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.048 &0.034 &0.041& 0.032 &0.039&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.076 &0.042& 0.029 &0.040 &0.042&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\midrule
&\multicolumn{10}{c}{GARCH noise}\\
&\multicolumn{5}{c}{$\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N\backslash T$&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&0.053 & 0.043 & 0.027 & 0.033 & 0.041 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
200& 0.079& 0.037 & 0.041 & 0.025 & 0.018 && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
500& 0.087 & 0.036 &0.037  & 0.034 &0.045  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
\bottomrule
\end{tabular}


==> Tables/tab_derand_GaussMain_secondround.tex <==
\centering
\begin{tabular}{ll|ccccccccccccccc}
\toprule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&1000&2000&&100&200&300&400&500&1000&2000\\
\midrule
100&LIL&0.067 & 0.011 & 0.001 & 0.000 & 0.000 &0.000&0.000
  && 0.962 & 0.976 & 0.982 & 0.984 & 0.989&&\\
& $f(B)=B^{-1/4}$ &0.004 & 0.000 & 0.000 & 0.000 & 0.000 &&
  && 0.930 & 0.958 & 0.971 & 0.972 & 0.975&&\\
200&LIL&0.059 & 0.006 & 0.000 & 0.000 & 0.000 &&
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000&&\\
& $f(B)=B^{-1/4}$ &0.010 & 0.000 & 0.000 & 0.000 & 0.000 &&
  && 0.996 & 0.997 & 0.999 & 1.000 & 1.000&&\\
500&LIL&0.381 & 0.224 & 0.162 & 0.104 & 0.077 &0.040&0.003
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000&&\\
& $f(B)=B^{-1/4}$ &0.012 & 0.000 & 0.000 & 0.000 & 0.000 &0.000&0.000
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000&&\\
\bottomrule
\end{tabular}


==> Tables/tab_derandomized_GARCH.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.016 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.969 & 0.980 & 0.984 & 0.985 & 0.989\\
& $f(B)=B^{-1/4}$ &0.000 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.969 & 0.980 & 0.984 & 0.985 & 0.989\\
200&LIL&0.009 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.002 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
500&LIL&0.276 & 0.137 & 0.080 & 0.050 & 0.028
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.001 & 0.000 & 0.000 & 0.000 & 0.000
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.067 & 0.011 & 0.001 & 0.000 & 0.000 
  && 0.962 & 0.976 & 0.982 & 0.984 & 0.989\\
& $f(B)=B^{-1/4}$ &0.004 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.930 & 0.958 & 0.971 & 0.972 & 0.975\\
200&LIL&0.059 & 0.006 & 0.000 & 0.000 & 0.000 
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.010 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.996 & 0.997 & 0.999 & 1.000 & 1.000\\
500&LIL&0.381 & 0.224 & 0.162 & 0.104 & 0.077 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.012 & 0.000 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\bottomrule
\end{tabular}


==> Tables/tab_derandomized_Gaussian.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.016 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.969 & 0.980 & 0.984 & 0.985 & 0.989\\
& $f(B)=B^{-1/4}$ &0.000 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.969 & 0.980 & 0.984 & 0.985 & 0.989\\
200&LIL&0.009 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.002 & 0.000 & 0.000 & 0.000 & 0.000
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
500&LIL&0.276 & 0.137 & 0.080 & 0.050 & 0.028
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.001 & 0.000 & 0.000 & 0.000 & 0.000
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.067 & 0.011 & 0.001 & 0.000 & 0.000 
  && 0.962 & 0.976 & 0.982 & 0.984 & 0.989\\
& $f(B)=B^{-1/4}$ &0.004 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.930 & 0.958 & 0.971 & 0.972 & 0.975\\
200&LIL&0.059 & 0.006 & 0.000 & 0.000 & 0.000 
  && 0.999 & 0.999 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.010 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.996 & 0.997 & 0.999 & 1.000 & 1.000\\
500&LIL&0.381 & 0.224 & 0.162 & 0.104 & 0.077 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
& $f(B)=B^{-1/4}$ &0.012 & 0.000 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\bottomrule
\end{tabular}


==> Tables/tab_derandomized_T.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.016 & 0.002 & 0.001 & 0.000 & 0.000 
  && 0.948 & 0.968 & 0.977 & 0.982 & 0.982\\
&$f(B) = B^{-1/4}$&0.001 & 0.001 & 0.000 & 0.000 & 0.000 
  && 0.895 & 0.935 & 0.952 & 0.964 & 0.972\\
200&LIL&0.016 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.996 & 0.997 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.000 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.988 & 0.994 & 0.996 & 0.997 & 0.998\\
500&LIL&0.356 & 0.137 & 0.093 & 0.065 & 0.039 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.003 & 0.001 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.056 & 0.007 & 0.001 & 0.000 & 0.000 
  && 0.945 & 0.966 & 0.974 & 0.981 & 0.983\\
&$f(B) = B^{-1/4}$&0.003 & 0.001 & 0.000 & 0.000 & 0.000 
  && 0.885 & 0.927 & 0.946 & 0.957 & 0.971\\
200&LIL&0.040 & 0.001 & 0.000 & 0.000 & 0.000 
  && 0.996 & 0.997 & 0.999 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.004 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.985 & 0.994 & 0.995 & 0.996 & 0.998\\
500&LIL&0.433 & 0.230 & 0.140 & 0.108 & 0.078 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.013 & 0.001 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\bottomrule
\end{tabular}


==> Tables/tab_derandomized_newGarch.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.026 & 0.003 & 0.000 & 0.000 & 0.000 
  && 0.985 & 0.989 & 0.995 & 0.996 & 0.995\\
&$f(B) = B^{-1/4}$&0.002 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.965 & 0.978 & 0.988 & 0.988 & 0.993\\
200&LIL&0.036 & 0.002 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.004 & 0.000 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
500&LIL&0.370 & 0.142 & 0.088 & 0.060 & 0.039 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.018 & 0.002 & 0.000 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{g} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{C.V. }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&LIL&0.085 & 0.013 & 0.003 & 0.000 & 0.001 
  && 0.983 & 0.986 & 0.994 & 0.996 & 0.995\\
&$f(B) = B^{-1/4}$&0.010 & 0.002 & 0.000 & 0.000 & 0.000 
  && 0.956 & 0.975 & 0.979 & 0.984 & 0.988\\
200&LIL&0.093 & 0.016 & 0.005 & 0.002 & 0.001 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.019 & 0.000 & 0.000 & 0.000 & 0.000 
  && 0.999 & 1.000 & 1.000 & 1.000 & 1.000\\
500&LIL&0.474 & 0.276 & 0.178 & 0.137 & 0.094 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
&$f(B) = B^{-1/4}$&0.059 & 0.005 & 0.001 & 0.000 & 0.000 
  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
\bottomrule
\end{tabular}


==> Tables/tab_size_Gaussian_experiment35.tex <==
%\centering
\begin{tabular}{ll|ccccccccccccccc}
\toprule
&&\multicolumn{7}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{7}{c}{$\phi_{g} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&1000&2000&&100&200&300&400&500&1000&2000\\
\midrule
100&Thm. 1 & 0.058 & 0.042 & 0.040 & 0.040 & 0.039 &0.040 &0.037 && 0.935 & 0.960 & 0.969 & 0.972 & 0.975 & & \\ 
&FLLM&0.124&0.112&0.101&0.088&0.095& & &&0.986&0.995&0.996&0.998&0.998 & & \\
&GRS& -- &0.053& 0.0345&0.045&0.047& & && -- & 0.994&  0.995&0.998&0.999\\
&FLY&0.353&0.218&0.150&0.129&0.138& &&&0.996&0.997&0.998&1.000&1.000\\ 
&GOS&0.212&0.200&0.179&0.185&0.193& &&&0.792&0.945&0.970&0.979&0.988\\
&PY&0.215&0.195&0.178&0.183&0.191& &&&0.785&0.941&0.970&0.979&0.988\\
&AS&0.104&0.075&0.066&0.077&0.089& &&&0.222&0.547&0.852&0.959&0.976\\
200&Thm. 1&0.071 & 0.039 & 0.036 & 0.036 & 0.035&0.034 &0.032 && 0.997 & 0.999 & 1.000 & 1.000 & 1.000\\ 
&FLLM&0.151&0.087&0.099&0.102&0.104 & & &&1.000&1.000&1.000&1.000&1.000& & \\
&GRS& -- & --&0.048&0.042&0.041&& --& -- &1.000&1.000&1.000  & & \\
&FLY&0.386&0.181&0.153&0.125&0.117& & &&1.000&1.000&1.000&1.000&1.000& & \\
&GOS&0.214&0.176&0.183&0.186&0.217& & &&0.863&0.987&0.995&0.999&1.000& & \\
&PY&0.219&0.174&0.182&0.185&0.217& & &&0.865&0.986&0.995&0.999&1.000& & \\
&AS&0.113&0.083&0.085&0.082&0.078& & &&0.225&0.657&0.944&0.995&0.999& & \\
500&Thm. 1&0.070 & 0.046 & 0.040 & 0.038 & 0.038& &  && 1.000 & 1.000 & 1.000 & 1.000 & 1.000& & \\
&FLLM&0.121&0.134&0.120&0.109&0.089 & &&&1.000&1.000&1.000&1.000&1.000 & &\\
&GRS& -- & -- & -- & -- & --&--&--&&--&--&--&--&--&--&--\\
&FLY&0.458&0.268&0.190&0.141&0.125& & &&1.000&1.000&1.000&1.000&1.000& & \\
&GOS&0.181&0.222&0.224&0.213&0.192& & &&0.936&1.000&1.000&1.000&1.000& & \\
&PY&0.192&0.220&0.221&0.212&0.191& &&&0.946&1.000&1.000&1.000&1.000& & \\
&AS&0.100&0.106&0.112&0.099&0.102& &&&0.248&0.768&0.979&0.999&1.000& & \\
\bottomrule
\end{tabular}


==> Tables/tab_size_T_experiment35.tex <==
\centering
\begin{tabular}{ll|ccccccccccccccc}
\toprule
&&\multicolumn{7}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{7}{c}{$\phi_{g} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&1000&2000&&100&200&300&400&500&1000&2000\\
\midrule
100&Thm. 1&0.058 & 0.046 & 0.039 & 0.037 & 0.038 &&&& 0.888 & 0.930 & 0.947 & 0.956 & 0.963&&\\
&FLLM&0.125&0.094&0.102&0.103&0.100&&&&0.977&0.992&0.999&1.000&1.000&&\\ 
& GRS & -- &0.043&0.044&0.035&0.051 &&&& -- & 0.991 & 0.996 & 0.998 & 0.999  &&\\
&FLY&0.337&0.175&0.139&0.118&0.113&&&&0.996&0.999&1.000&1.000&1.000&&\\
&GOS&0.000&0.000&0.000&0.000&0.000&&&&0.794&0.934&0.973&0.983&0.991&&\\
&PY&0.242&0.196&0.202&0.198&0.208&&&&0.826&0.934&0.973&0.983&0.991&&\\
&AS&0.093&0.079&0.088&0.079&0.088&&&&0.170&0.474&0.798&0.934&0.965&&\\
200&Thm. 1&0.056 & 0.040 & 0.037 & 0.037 & 0.035 &&&& 0.982 & 0.993 & 0.997 & 0.997 & 0.998&&\\
&FLLM&0.104&0.114&0.108&0.109&0.110&&&&0.999&1.000&1.000&1.000&1.000&&\\ 
& GRS & -- & -- & 0.062&0.060&0.044 &&&& -- &--& 1.000&1.000&1.000 &&\\
&FLY&0.379&0.228&0.156&0.139&0.119&&&&1.000&1.000&1.000&1.000&1.000&&\\ 
&GOS&0.000&0.000&0.000&0.202&0.219&&&&0.858&0.980&0.993&0.998&1.000&&\\
&PY&0.240&0.217&0.197&0.201&0.217&&&&0.891&0.979&0.993&0.998&1.000&&\\
&AS&0.102&0.077&0.082&0.101&0.096&&&&0.192&0.553&0.904&0.989&0.993&&\\
500&Thm. 1&0.068 & 0.039 & 0.038 & 0.040 & 0.039 &&&& 1.000 & 1.000 & 1.000 & 1.000 & 1.000&&\\
&FLLM&0.135&0.103&0.123&0.114&0.111&&&&1.000&1.000&1.000&1.000&1.000&&\\
&GRS& -- & -- & -- & -- & --&&&& -- & -- & -- & -- & --&&\\
&FLY&0.488&0.232&0.177&0.138&0.132&&&&1.000&1.000&1.000&1.000&1.000&&\\
&GOS&0.271&0.211&0.203&0.206&0.211&&&&0.942&0.998&1.000&1.000&1.000&&\\
&PY&0.270&0.209&0.201&0.204&0.207&&&&0.969&0.999&1.000&1.000&1.000&&\\
&AS&0.097&0.085&0.099&0.095&0.108&&&&0.223&0.637&0.966&0.996&0.999&&\\
\bottomrule
\end{tabular}


==> Tables/tab_size_T_numezzi.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.042&0.033&0.032&0.032&0.032&&0.997&1.000&1.000&1.000&1.000\\
&nu/2&0.041&0.029&0.034&0.034&0.034&&0.362&0.526&0.712&0.816&0.889\\
&FLLM&0.052&0.033&0.036&0.032&0.037&&1.000&1.000&1.000&1.000&1.000\\
200&nu&0.059&0.041&0.041&0.040&0.040&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.049&0.036&0.041&0.035&0.032&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.043&0.048&0.032&0.038&0.040&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.072&0.044&0.039&0.038&0.038&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.038&0.054&0.033&0.033&0.033&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.053&0.038&0.041&0.037&0.042&&1.000&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.067&0.036&0.033&0.032&0.032&&0.996&1.000&1.000&1.000&1.000\\
&nu/2&0.056&0.042&0.032&0.031&0.036&&0.896&0.989&1.000&1.000&1.000\\
&FLLM&0.125&0.094&0.102&0.103&0.100&&1.000&1.000&1.000&1.000&1.000\\
200&nu&0.081&0.041&0.041&0.040&0.040&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.053&0.041&0.038&0.035&0.043&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.104&0.114&0.108&0.109&0.110&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.109&0.045&0.039&0.038&0.038&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.069&0.053&0.034&0.040&0.034&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.135&0.103&0.123&0.114&0.111&&1.000&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.265&0.119&0.077&0.059&0.051&&0.923&0.974&0.996&1.000&1.000\\
&nu/2&0.218&0.111&0.078&0.055&0.061&&0.794&0.801&0.892&0.955&0.972\\
&FLLM&0.394&0.378&0.372&0.367&0.379&&0.986&1.000&1.000&1.000&1.000\\
200&nu&0.293&0.151&0.088&0.073&0.062&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.217&0.110&0.081&0.085&0.049&&0.988&1.000&1.000&1.000&1.000\\
&FLLM&0.379&0.391&0.372&0.370&0.367&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.330&0.172&0.111&0.078&0.065&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.257&0.130&0.121&0.085&0.067&&1.000&1.000&1.000&1.000&1.000\\
50&FLLM&0.384&0.376&0.373&0.374&0.375&&1.000&1.000&1.000&1.000&1.000\\
\bottomrule
\end{tabular}










==> Tables/tab_size_garch.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300&400&500&&100&200&300&400&500\\
\midrule
100&Thm. 1&0.056 & 0.043 & 0.040 & 0.039 & 0.039 && 0.967 & 0.983 & 0.989 & 0.99 & 0.992\\
&FLLM&0.045&0.045&0.035&0.023&0.024&&0.988&0.995&0.997&0.998&0.998\\
&FLY&0.209&0.109&0.096&0.098&0.088&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.081&0.071&0.063&0.057&0.065&&0.805&0.946&0.976&0.982&0.992\\
&PY&0.087&0.068&0.060&0.055&0.065&&0.810&0.946&0.976&0.982&0.992\\
&AS&0.068&0.069&0.064&0.061&0.072&&0.219&0.685&0.941&0.988&0.992\\
200&Thm. 1&0.048 & 0.035 & 0.033 & 0.032 & 0.032 && 1.000 & 1.000 & 1.000 & 1.00 & 1.000\\
&FLLM&0.055&0.027&0.027&0.028&0.028&&1.000&1.000&1.000&1.000&1.000\\
&FLY&0.234&0.139&0.104&0.091&0.085&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.088&0.062&0.064&0.065&0.061&&0.888&0.986&0.997&0.999&1.000\\
&PY&0.096&0.059&0.062&0.064&0.061&&0.902&0.986&0.997&0.999&1.000\\
&AS&0.079&0.059&0.080&0.078&0.082&&0.253&0.833&0.984&1.000&1.000\\
500&Thm. 1&0.065 & 0.041 & 0.035 & 0.036 & 0.035 && 1.000 & 1.000 & 1.000 & 1.00 & 1.000\\
&FLLM&0.035&0.044&0.036&0.027&0.029&&1.000&1.000&1.000&1.000&1.000\\
&FLY&0.388&0.189&0.129&0.100&0.083&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.071&0.084&0.087&0.078&0.068&&0.951&1.000&1.000&1.000&1.000\\
&PY&0.082&0.083&0.085&0.077&0.067&&0.973&1.000&1.000&1.000&1.000\\
&AS&0.069&0.089&0.099&0.084&0.090&&0.291&0.913&0.999&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&Thm. 1&0.079 & 0.050 & 0.044 & 0.042 & 0.040 && 0.965 & 0.975 & 0.98 & 0.987 & 0.987\\
&FLLM&0.124&0.112&0.101&0.088&0.095&&0.986&0.995&0.996&0.998&0.998\\
&FLY&0.313&0.174&0.154&0.135&0.123&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.212&0.200&0.179&0.185&0.193&&0.792&0.945&0.970&0.979&0.988\\
&PY&0.215&0.195&0.178&0.183&0.191&&0.785&0.941&0.970&0.979&0.988\\
&AS&0.104&0.075&0.066&0.077&0.089&&0.222&0.547&0.852&0.959&0.976\\
200&Thm. 1&0.070 & 0.042 & 0.036 & 0.033 & 0.034 && 1.000 & 1.000 & 1.00 & 1.000 & 1.000\\
&FLLM&0.151&0.087&0.099&0.102&0.104&&1.000&1.000&1.000&1.000&1.000\\
&FLY&0.315&0.212&0.144&0.136&0.120&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.214&0.176&0.183&0.186&0.217&&0.863&0.987&0.995&0.999&1.000\\
&PY&0.219&0.174&0.182&0.185&0.217&&0.865&0.986&0.995&0.999&1.000\\
&AS&0.113&0.083&0.085&0.082&0.078&&0.225&0.657&0.944&0.995&0.999\\
500&Thm. 1&0.109 & 0.053 & 0.043 & 0.038 & 0.039 && 1.000 & 1.000 & 1.00 & 1.000 & 1.000\\
&FLLM&0.121&0.134&0.120&0.109&0.089&&1.000&1.000&1.000&1.000&1.000\\
&FLY&0.471&0.247&0.165&0.132&0.103&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.181&0.222&0.224&0.213&0.192&&0.936&1.000&1.000&1.000&1.000\\
&PY&0.192&0.220&0.221&0.212&0.191&&0.946&1.000&1.000&1.000&1.000\\
&AS&0.100&0.106&0.112&0.099&0.102&&0.248&0.768&0.979&0.999&1.000\\
\bottomrule
\end{tabular}


==> Tables/tab_size_garch_numezzi.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.138&0.057&0.035&0.033&0.033&&0.756&0.939&0.985&0.994&0.998\\
&nu/2&0.061&0.043&0.023&0.041&0.038&&0.362&0.526&0.712&0.816&0.889\\
&FLLM&0.053&0.049&0.048&0.037&0.050&&0.871&0.977&0.994&0.998&0.998\\
200&nu&0.227&0.084&0.057&0.043&0.041&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.108&0.037&0.034&0.048&0.035&&0.988&1.000&1.000&1.000&1.000\\
&FLLM&0.062&0.056&0.046&0.047&0.039&&0.989&1.000&1.000&1.000&1.000\\
500&nu&0.445&0.133&0.082&0.053&0.048&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.165&0.057&0.053&0.032&0.038&&0.999&1.000&1.000&1.000&1.000\\
&FLLM&0.069&0.061&0.061&0.050&0.045&&0.999&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.148&0.058&0.037&0.033&0.033&&0.736&0.920&0.977&0.992&0.997\\
&nu/2&0.074&0.042&0.038&0.027&0.031&&0.352&0.510&0.687&0.785&0.874\\
&FLLM&0.117&0.095&0.098&0.089&0.096&&0.870&0.977&0.995&0.998&0.998\\
200&nu&0.242&0.087&0.056&0.044&0.041&&0.999&1.000&1.000&1.000&1.000\\
&nu/2&0.096&0.053&0.037&0.036&0.035&&0.984&0.999&1.000&1.000&1.000\\
&FLLM&0.111&0.113&0.104&0.108&0.094&&0.989&1.000&1.000&1.000&1.000\\
500&nu&0.478&0.139&0.085&0.055&0.047&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.183&0.065&0.044&0.038&0.042&&0.996&1.000&1.000&1.000&1.000\\
&FLLM&0.128&0.114&0.110&0.109&0.102&&1.000&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.309&0.119&0.074&0.050&0.042&&0.694&0.771&0.863&0.925&0.952\\
&nu/2&0.182&0.082&0.055&0.031&0.044&&0.394&0.434&0.512&0.606&0.659\\
&FLLM&0.390&0.364&0.367&0.362&0.368&&0.872&0.972&0.993&0.998&0.999\\
200&nu&0.397&0.169&0.100&0.067&0.050&&0.998&1.000&1.000&1.000&1.000\\
&nu/2&0.191&0.076&0.065&0.046&0.040&&0.929&0.987&0.998&0.999&0.999\\
&FLLM&0.364&0.367&0.360&0.373&0.368&&0.994&1.000&1.000&1.000&1.000\\
500&nu&0.599&0.272&0.129&0.092&0.066&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.299&0.110&0.071&0.042&0.050&&0.976&0.996&0.999&1.000&1.000\\
&FLLM&0.410&0.405&0.381&0.378&0.353&&0.998&1.000&1.000&1.000&1.000\\
\bottomrule
\end{tabular}























==> Tables/tab_size_gaussian_numezzi.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} = 0$ for all $i$} &&\multicolumn{5}{c}{$\phi_{\nu} = 0$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.039&0.032&0.032&0.032&0.033&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.039&0.043&0.034&0.027&0.037&&0.998&1.000&1.000&1.000&1.000\\
&FLLM&0.045&0.045&0.035&0.023&0.024&&1.000&1.000&1.000&1.000&1.000\\
200&nu&0.046&0.040&0.040&0.040&0.040&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.044&0.035&0.041&0.041&0.041&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.055&0.027&0.027&0.028&0.028&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.051&0.038&0.038&0.038&0.038&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.049&0.037&0.050&0.033&0.021&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.035&0.044&0.036&0.027&0.029&&1.000&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.066&0.035&0.033&0.033&0.033&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.069&0.045&0.034&0.022&0.037&&0.987&1.000&1.000&1.000&1.000\\
&FLLM&0.124&0.112&0.101&0.088&0.095&&1.000&1.000&1.000&1.000&1.000\\
200&nu&0.081&0.043&0.040&0.040&0.040&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.068&0.032&0.046&0.022&0.032&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.151&0.087&0.099&0.102&0.104&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.086&0.042&0.039&0.039&0.040&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.068&0.055&0.046&0.032&0.040&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.121&0.134&0.120&0.109&0.089&&1.000&1.000&1.000&1.000&1.000\\
\midrule
&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{\nu} = 0.8$; $\alpha_{i} \sim N(0,1)$ for 1\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&nu&0.277&0.142&0.089&0.069&0.062&&0.969&0.990&1.000&1.000&1.000\\
&nu/2&0.228&0.127&0.095&0.069&0.049&&0.867&0.939&0.980&0.990&0.995\\
&FLLM&0.386&0.354&0.346&0.338&0.337&&0.995&1.000&1.000&1.000&1.000\\
200&nu&0.322&0.149&0.107&0.084&0.070&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.263&0.138&0.093&0.084&0.061&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.399&0.340&0.327&0.329&0.348&&1.000&1.000&1.000&1.000&1.000\\
500&nu&0.318&0.196&0.133&0.103&0.077&&1.000&1.000&1.000&1.000&1.000\\
&nu/2&0.275&0.178&0.140&0.099&0.070&&1.000&1.000&1.000&1.000&1.000\\
&FLLM&0.366&0.365&0.378&0.338&0.352&&1.000&1.000&1.000&1.000&1.000\\
\bottomrule
\end{tabular}
























==> Tables/tab_size_newGarch_experiment35.tex <==
\centering
\begin{tabular}{ll|ccccccccccc}
\toprule
&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} = 0$ for all $i$}&&\multicolumn{5}{c}{$\phi_{g} = 0.4$; $\alpha_{i} \sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash$T&100&200&300& 400&500&&100&200&300&400&500\\
\midrule
100&Thm. 1&0.079 & 0.050 & 0.044 & 0.042 & 0.040 && 0.965 & 0.975 & 0.98 & 0.987 & 0.987\\
&FLLM&0.124&0.112&0.101&0.088&0.095&&0.986&0.995&0.996&0.998&0.998\\
& GRS  &--&0.046 &0.046 &0.047 &0.035&&--&0.999&0.999&0.999&0.999\\
&FLY&0.313&0.174&0.154&0.135&0.123&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.212&0.200&0.179&0.185&0.193&&0.792&0.945&0.970&0.979&0.988\\
&PY&0.215&0.195&0.178&0.183&0.191&&0.785&0.941&0.970&0.979&0.988\\
&AS&0.104&0.075&0.066&0.077&0.089&&0.222&0.547&0.852&0.959&0.976\\
200&Thm. 1&0.070 & 0.042 & 0.036 & 0.033 & 0.034 && 1.000 & 1.000 & 1.00 & 1.000 & 1.000\\
&FLLM&0.151&0.087&0.099&0.102&0.104&&1.000&1.000&1.000&1.000&1.000\\
& GRS &--&-- &0.057&0.062&0.051&&--&--&1.000&1.000&1.000\\
&FLY&0.315&0.212&0.144&0.136&0.120&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.214&0.176&0.183&0.186&0.217&&0.863&0.987&0.995&0.999&1.000\\
&PY&0.219&0.174&0.182&0.185&0.217&&0.865&0.986&0.995&0.999&1.000\\
&AS&0.113&0.083&0.085&0.082&0.078&&0.225&0.657&0.944&0.995&0.999\\
500&Thm. 1&0.109 & 0.053 & 0.043 & 0.038 & 0.039 && 1.000 & 1.000 & 1.00 & 1.000 & 1.000\\
&FLLM&0.121&0.134&0.120&0.109&0.089&&1.000&1.000&1.000&1.000&1.000\\
& GRS -- & -- &--&--&--&& -- & -- &-- & -- & -- \\
&FLY&0.471&0.247&0.165&0.132&0.103&&1.000&1.000&1.000&1.000&1.000\\
&GOS&0.181&0.222&0.224&0.213&0.192&&0.936&1.000&1.000&1.000&1.000\\
&PY&0.192&0.220&0.221&0.212&0.191&&0.946&1.000&1.000&1.000&1.000&1.000&1.000\\
&AS&0.100&0.106&0.112&0.099&0.102&&0.248&0.768&0.979&0.999&1.000\\
\bottomrule
\end{tabular}


==> Tables/table_MCempirical.tex <==
\centering
\begin{tabular}{l|cccccccccc}
\toprule
$N\backslash \sigma_{\varepsilon}$&1&2&3&4&5&6&7&8&9&10\\
\midrule
Thm1 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.999 & 0.999 & 1.000 & 1.000 & 1.000 \\
FLLM & 1.000 & 1.000 & 0.993 & 0.918 & 0.748 & 0.539 & 0.385 & 0.295 & 0.245 & 0.213 \\
PY & 0.793 & 0.411 & 0.299 & 0.265 & 0.247 & 0.240 & 0.235 & 0.228 & 0.227 & 0.227 \\
GOS & 0.764 & 0.544 & 0.660 & 0.552 & 0.512 & 0.485 & 0.475 & 0.463 & 0.457 & 0.454 \\
AS & 0.220 & 0.172 & 0.136 & 0.121 & 0.115 & 0.110 & 0.105 & 0.109 & 0.104 & 0.105 \\
FLY & 1.000 & 1.000 & 1.000 & 0.993 & 0.969 & 0.915 & 0.843 & 0.742 & 0.647 & 0.542 \\
\bottomrule
\end{tabular}


==> tab_size_T_weakOmitted.tex <==
\centering
\begin{tabular}{ll|
                S S S S S S
                c
                S S S S S S}
\toprule
&&\multicolumn{6}{c}{$\phi_g=0$; $\alpha_i=0$ for all $i$}&&
  \multicolumn{6}{c}{$\phi_g=0$; $\alpha_i\sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash T$
&{100}&{200}&{300}&{500}&{1000}&{2000}&&
 {100}&{200}&{300}&{500}&{1000}&{2000}\\
\midrule
100&Thm.\ 1
&4.0&2.7&3.5&3.3&3.2&3.2&&
 94.1&95.9&96.8&98.0&99.4&99.7\\
&FLLM
&4.8&5.7&4.4&3.4&4.4&5.3&&
 98.4&99.8&99.9&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&4.5&4.7&3.4&3.6&2.7&&
 \multicolumn{1}{c}{--}&98.5&99.7&99.9&100.0&100.0\\
&FLY
&27.9&16.8&11.4&7.4&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.0&99.8&99.9&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&8.4&6.9&6.3&5.7&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 98.3&99.4&99.8&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&6.3&5.3&5.8&5.3&5.5&5.9&&
 98.1&99.4&99.7&100.0&100.0&100.0\\
&AS
&5.0&5.3&6.4&5.9&5.2&5.5&&
 15.3&51.3&88.1&98.5&100.0&100.0\\
\midrule
200&Thm.\ 1
&5.1&3.5&4.0&3.0&4.2&4.0&&
 99.6&99.9&100.0&100.0&100.0&100.0\\
&FLLM
&6.1&4.6&3.2&5.4&4.6&4.4&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&3.9&4.6&3.8&3.8&&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&100.0&100.0&100.0&100.0\\
&FLY
&32.5&14.6&10.7&8.5&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 100.0&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&9.3&7.4&6.0&6.6&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.6&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&6.1&5.7&5.2&5.9&6.4&4.9&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&AS
&6.2&5.8&5.5&5.9&5.9&6.1&&
 16.3&64.3&96.5&99.9&100.0&100.0\\
\midrule
500&Thm.\ 1
&3.0&5.4&3.1&3.1&4.2&3.9&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&FLLM
&7.1&5.1&4.9&4.3&3.6&2.6&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&4.5&5.1&&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&100.0&100.0\\
&FLY
&43.1&17.3&12.2&8.4&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 100.0&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&9.9&6.4&6.2&5.3&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.3&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&4.4&4.6&5.0&4.8&4.8&4.2&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&AS
&4.6&4.3&5.0&5.4&4.8&5.4&&
 17.7&80.7&99.4&100.0&100.0&100.0\\
\midrule
&&\multicolumn{6}{c}{$\phi_g=0.4$; $\alpha_i=0$ for all $i$}&&
  \multicolumn{6}{c}{$\phi_g=0.4$; $\alpha_i\sim N(0,1)$ for 5\% of units} \\
\midrule
$N$&$\text{Test }\backslash T$
&{100}&{200}&{300}&{500}&{1000}&{2000}&&
 {100}&{200}&{300}&{500}&{1000}&{2000}\\
\midrule
100&Thm.\ 1
&4.8&3.6&2.8&3.5&3.2&3.2&&
 94.4&96.3&97.1&97.8&99.4&99.7\\
&FLLM
&5.5&6.8&5.6&4.6&6.1&7.0&&
 98.4&99.9&100.0&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&5.1&4.9&4.0&4.3&3.6&&
 \multicolumn{1}{c}{--}&98.4&99.7&99.9&100.0&100.0\\
&FLY
&31.3&19.0&13.3&8.5&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.0&99.9&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&12.0&11.0&8.9&8.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 98.4&99.5&99.7&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&8.8&8.9&8.2&7.4&7.8&9.3&&
 98.3&99.4&99.7&100.0&100.0&100.0\\
&AS
&4.5&5.6&6.5&5.9&5.4&5.5&&
 15.3&51.2&87.4&98.4&100.0&100.0\\
\midrule
200&Thm.\ 1
&3.8&4.0&3.5&4.0&4.2&4.0&&
 99.7&99.9&100.0&100.0&100.0&100.0\\
&FLLM
&7.0&5.3&4.4&6.3&5.3&5.3&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&4.7&4.7&4.5&4.4&&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&100.0&100.0&100.0&100.0\\
&FLY
&34.6&17.0&12.3&10.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 100.0&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&12.0&9.7&8.8&9.6&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.6&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&8.2&8.0&7.9&9.1&8.2&7.0&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&AS
&6.4&5.8&5.5&5.8&5.9&6.0&&
 17.0&64.8&96.3&99.9&100.0&100.0\\
\midrule
500&Thm.\ 1
&5.1&5.0&3.6&3.0&4.2&3.9&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&FLLM
&7.3&5.9&5.0&4.5&4.4&3.2&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&GRS
&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&4.9&5.5&&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&100.0&100.0\\
&FLY
&46.9&19.2&14.1&9.6&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 100.0&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&GOS
&12.2&8.8&7.9&7.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&&
 99.3&100.0&100.0&100.0&
 \multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}\\
&PY
&6.5&5.9&6.1&6.5&7.4&6.7&&
 100.0&100.0&100.0&100.0&100.0&100.0\\
&AS
&4.9&4.2&4.9&5.2&4.9&5.5&&
 17.8&80.9&99.4&100.0&100.0&100.0\\
\bottomrule
\end{tabular}

